Reconfigurable Intelligent Surface for Industrial Automation: mmWave Propagation Measurement, Simulation, and Control Algorithm Requirements

Reconfigurable intelligent surfaces (RISs) enable reliable low-latency millimeter wave (mmWave) communication links in cases of a blocked line-of-sight (LoS) between the base station (BS) and the user equipment (UE), i.e. a RIS mounted on a wall or the ceiling provides a bypass for the radio communication link. We present an active RIS with 127 patch antenna elements arranged in a hexagonal grid for a center frequency of 23.8 GHz. Each RIS element uses an orthogonal polarization transformation to enable amplification using a field-effect transistor (FET). The source and drain voltages of each FET is controlled using two bits. We assume that the coordinates of the UE in an industrial control scenario are known to the RIS. We measure the received power on a 2D grid of 60 cm by 100 cm with the RIS working in reflective and active mode. The results show that the RIS can successfully focus the radio signal at the desired target points. The half-power beam width is characterized in axial and radial directions with respect to the RIS position, obtaining a practical RIS configuration update criterion for a mobile UE. These results clearly show that RISs are prominent solutions for enabling reliable wireless communication in indoor industrial scenarios.

==> cqhhngczbkvcxbfzrqfmzkzsrhpmvgtx/abbrev.tex <==
\begin{acronym} 
\setlength{\itemsep}{-0.63\parsep}
\acro{3GPP}{3rd Generation Partnership Project}
%\acro{AOA}{angle of arrival}
%\acro{AOD}{angle of departure}
\acro{ACF}{auto correlation function}
%\acro{ASIC}{application-specific integrated circuit}
\acro{ADC}{analog-to-digital converter}
%\acro{AWGN}{additive white Gaussian noise}
\acro{BEM}{basis-expansion model}
%\acro{BLER}{block error rate}
%\acro{BER}{bit-error-rate}
%\acro{CA}{complex addition}
\acro{CDF}{cumulative distribution function}
\acro{CE}{complex exponential}
\acro{CIR}{channel impulse response}
%\acro{CDMA}{code division multiple access}
%\acro{CM}{complex multiplication}
%\acro{COTS}{common-off-the-shelf}
\acro{CP}[CP]{cyclic prefix}
%\acro{CSM}{complex scalar multiplication}
\acro{CTF}{channel transfer function}
\acro{D2D}{device-to-device}
\acro{DAC}{digital-to-analog converter}
\acro{DC}{direct current}
%\acro{DDC}{direct down conversion}
%\acro{DMA}{direct memory access}
\acro{DOD}{direction of departure}
\acro{DOA}{direction of arrival}
%\acro{DUC}{direct up conversion}
\acro{DPS}{discrete prolate spheroidal}
\acro{DPSWF}{discrete prolate spheroidal wave function}
\acro{DSD}{Doppler spectral density}
\acro{DSP}{digital signal processor}
\acro{DR}{dynamic range}
%\acro{eNodeB}{base station}
%\acro{eMBB}{enhanced mobile broadband} %used
\acro{ETSI}{European Telecommunications Standards Institute}
%\acro{FER}{frame error rate}
\acro{FIFO}{first-input first-output}
\acro{FFT}{fast Fourier transform}
%\acro{FLOPS}{floating point operations per second}
\acro{FP}{fixed-point}
\acro{FPGA}{field programmable gate array}
%\acro{FPS}{frames per second}
%\acro{GCE}{geometry-based channel emulator}
\acro{GSCM}{geometry-based stochastic channel model}
%\acro{GCM}{geometry-based channel model}
\acro{GSM}{global system for mobile communications}
\acro{GPS}{global positioning system}
%\acro{HiL}{hardware-in-the-loop}
\acro{HPBW}{half power beam width}
\acro{ICI}[ICI]{inter-carrier interference}
\acro{IDFT}{inverse discrete Fourier transform}
\acro{IF}{intermediate frequency}
\acro{IFFT}{inverse fast Fourier transform}
\acro{ISI}{inter-symbol interference}
\acro{ITS}{intelligent transportation system}
%\acro{mMTC}{massive machine type communications} %used
%\acro{MAC}{multiply-accumulate}
\acro{MEC}{mobile edge computing}
\acro{MSE}{mean square error}
\acro{LLR}{log-likelihood ratio}
\acro{LO}{local oscillator}
\acro{LOS}{line-of-sight}
\acro{LMMSE}{linear minimum mean squared error}
\acro{LNA}{low noise amplifier}
\acro{LSF}{local scattering function}
\acro{LTE}{long term evolution}
%\acro{LTE-A}{Long Term Evolution Advanced}
\acro{LUT}{look-up table}
\acro{LTV}{linear time-variant }
\acro{MIMO}{multiple-input multiple-output}
\acro{MPC}{multi-path component}
\acro{MC}{Monte Carlo}
\acro{NI}{National Instruments}
\acro{LoS}{line-of-sight}
\acro{NLOS}{non-line of sight}
\acro{OFDM}{orthogonal frequency division multiplexing}
\acro{OTA}{over-the-air}
\acro{PA}{power amplifier}
\acro{PC}{personal computer}
\acro{PDP}{power delay profile}
%\acro{PDF}{probability density function}
\acro{PER}{packet error rate}
\acro{PPS}{pulse per second}
%\acro{P2P}{peer-to-peer}
\acro{QAM}{quadrature ampltiude modulation}
\acro{QPSK}{quadrature phase shift keying}

%\acro{UE}{user equipment}
\acro{RB}{resource block}
\acro{RBP}{resource block pair}
\acro{RIS}{reflective intelligent surface}
\acro{RF}{radio frequency}
\acro{RMS}{root mean square}
\acro{RSSI}{receive signal strength indicator}
\acro{RT}{ray tracing}
\acro{RX}{receiver}
\acro{SCME}{spatial channel model extended}
\acro{SDR}{software defined radio}
\acro{SISO}{single-input single-output}
\acro{SoCE}{sum of complex exponentials}
\acro{SNR}{signal-to-noise ratio}
\acro{SUT}{system-under test}
\acro{SSD}{soft sphere decoder}
\acro{TBWP}{time-bandwidth product}
\acro{TDL}{tap delay line}
%\acro{TTI}{transmission time intervall}
\acro{TX}{transmitter}
%\acro{UAV}{unmanned ariel vehicle}
\acro{UMTS}{universal mobile telecommunications systems}
\acro{UDP}{user datagram protocol}
\acro{URLLC}{ultra-reliable and low latency communication} %yes
\acro{US}{uncorrelated-scattering}
\acro{USRP}{universal software radio peripheral}
\acro{VNA}{vector network analyzer}
\acro{ViL}{vehicle-in-the-loop}
\acro{V2I}{vehicle-to-infrastructure}
\acro{V2V}{vehicle-to-vehicle}
\acro{V2X}{vehicle-to-everything}
\acro{VST}{vector signal transceiver}
\acro{VTD}{Virtual Test Drive}
\acro{WF}{Wiener filter}
\acro{WSS}{wide-sense-stationary}
\acro{WSSUS}{wide-sense-stationary uncorrelated-scattering}
\end{acronym}

==> pwvrkmpftpfnjtyktdpzxngnvtvngtxq/abbrev.tex <==
\begin{acronym} 
\setlength{\itemsep}{-0.63\parsep}
\acro{3GPP}{3rd Generation Partnership Project}
%\acro{AOA}{angle of arrival}
%\acro{AOD}{angle of departure}
\acro{ACF}{auto correlation function}
%\acro{ASIC}{application-specific integrated circuit}
\acro{ADC}{analog-to-digital converter}
%\acro{AWGN}{additive white Gaussian noise}
\acro{BEM}{basis-expansion model}
%\acro{BLER}{block error rate}
%\acro{BER}{bit-error-rate}
%\acro{CA}{complex addition}
\acro{CDF}{cumulative distribution function}
\acro{CE}{complex exponential}
\acro{CIR}{channel impulse response}
%\acro{CDMA}{code division multiple access}
%\acro{CM}{complex multiplication}
%\acro{COTS}{common-off-the-shelf}
\acro{CP}[CP]{cyclic prefix}
%\acro{CSM}{complex scalar multiplication}
\acro{CTF}{channel transfer function}
\acro{D2D}{device-to-device}
\acro{DAC}{digital-to-analog converter}
\acro{DC}{direct current}
%\acro{DDC}{direct down conversion}
%\acro{DMA}{direct memory access}
\acro{DOD}{direction of departure}
\acro{DOA}{direction of arrival}
%\acro{DUC}{direct up conversion}
\acro{DPS}{discrete prolate spheroidal}
\acro{DPSWF}{discrete prolate spheroidal wave function}
\acro{DSD}{Doppler spectral density}
\acro{DSP}{digital signal processor}
\acro{DR}{dynamic range}
%\acro{eNodeB}{base station}
%\acro{eMBB}{enhanced mobile broadband} %used
\acro{ETSI}{European Telecommunications Standards Institute}
%\acro{FER}{frame error rate}
\acro{FIFO}{first-input first-output}
\acro{FFT}{fast Fourier transform}
%\acro{FLOPS}{floating point operations per second}
\acro{FP}{fixed-point}
\acro{FPGA}{field programmable gate array}
%\acro{FPS}{frames per second}
%\acro{GCE}{geometry-based channel emulator}
\acro{GSCM}{geometry-based stochastic channel model}
%\acro{GCM}{geometry-based channel model}
\acro{GSM}{global system for mobile communications}
\acro{GPS}{global positioning system}
%\acro{HiL}{hardware-in-the-loop}
\acro{HPBW}{half power beam width}
\acro{ICI}[ICI]{inter-carrier interference}
\acro{IDFT}{inverse discrete Fourier transform}
\acro{IF}{intermediate frequency}
\acro{IFFT}{inverse fast Fourier transform}
\acro{ISI}{inter-symbol interference}
\acro{ITS}{intelligent transportation system}
%\acro{mMTC}{massive machine type communications} %used
%\acro{MAC}{multiply-accumulate}
\acro{MEC}{mobile edge computing}
\acro{MSE}{mean square error}
\acro{LLR}{log-likelihood ratio}
\acro{LO}{local oscillator}
\acro{LOS}{line-of-sight}
\acro{LMMSE}{linear minimum mean squared error}
\acro{LNA}{low noise amplifier}
\acro{LSF}{local scattering function}
\acro{LTE}{long term evolution}
%\acro{LTE-A}{Long Term Evolution Advanced}
\acro{LUT}{look-up table}
\acro{LTV}{linear time-variant }
\acro{MIMO}{multiple-input multiple-output}
\acro{MPC}{multi-path component}
\acro{MC}{Monte Carlo}
\acro{NI}{National Instruments}
\acro{LoS}{line-of-sight}
\acro{NLOS}{non-line of sight}
\acro{OFDM}{orthogonal frequency division multiplexing}
\acro{OTA}{over-the-air}
\acro{PA}{power amplifier}
\acro{PC}{personal computer}
\acro{PDP}{power delay profile}
%\acro{PDF}{probability density function}
\acro{PER}{packet error rate}
\acro{PPS}{pulse per second}
%\acro{P2P}{peer-to-peer}
\acro{QAM}{quadrature ampltiude modulation}
\acro{QPSK}{quadrature phase shift keying}

%\acro{UE}{user equipment}
\acro{RB}{resource block}
\acro{RBP}{resource block pair}
\acro{RIS}{reflective intelligent surface}
\acro{RF}{radio frequency}
\acro{RMS}{root mean square}
\acro{RSSI}{receive signal strength indicator}
\acro{RT}{ray tracing}
\acro{RX}{receiver}
\acro{SCME}{spatial channel model extended}
\acro{SDR}{software defined radio}
\acro{SISO}{single-input single-output}
\acro{SoCE}{sum of complex exponentials}
\acro{SNR}{signal-to-noise ratio}
\acro{SUT}{system-under test}
\acro{SSD}{soft sphere decoder}
\acro{TBWP}{time-bandwidth product}
\acro{TDL}{tap delay line}
%\acro{TTI}{transmission time intervall}
\acro{TX}{transmitter}
%\acro{UAV}{unmanned ariel vehicle}
\acro{UMTS}{universal mobile telecommunications systems}
\acro{UDP}{user datagram protocol}
\acro{URLLC}{ultra-reliable and low latency communication} %yes
\acro{US}{uncorrelated-scattering}
\acro{USRP}{universal software radio peripheral}
\acro{VNA}{vector network analyzer}
\acro{ViL}{vehicle-in-the-loop}
\acro{V2I}{vehicle-to-infrastructure}
\acro{V2V}{vehicle-to-vehicle}
\acro{V2X}{vehicle-to-everything}
\acro{VST}{vector signal transceiver}
\acro{VTD}{Virtual Test Drive}
\acro{WF}{Wiener filter}
\acro{WSS}{wide-sense-stationary}
\acro{WSSUS}{wide-sense-stationary uncorrelated-scattering}
\end{acronym}
